Certifiable Robustness for Nearest Neighbor Classifiers

ML models are typically trained using large datasets of high quality. However, training datasets often contain inconsistent or incomplete data. To tackle this issue, one solution is to develop algorithms that can check whether a prediction of a model is certifiably robust. Given a learning algorithm that produces a classifier and given an example at test time, a classification outcome is certifiably robust if it is predicted by every model trained across all possible worlds (repairs) of the uncertain (inconsistent) dataset. This notion of robustness falls naturally under the framework of certain answers. In this paper, we study the complexity of certifying robustness for a simple but widely deployed classification algorithm, $k$-Nearest Neighbors ($k$-NN). Our main focus is on inconsistent datasets when the integrity constraints are functional dependencies (FDs). For this setting, we establish a dichotomy in the complexity of certifying robustness w.r.t. the set of FDs: the problem either admits a polynomial time algorithm, or it is coNP-hard. Additionally, we exhibit a similar dichotomy for the counting version of the problem, where the goal is to count the number of possible worlds that predict a certain label. As a byproduct of our study, we also establish the complexity of a problem related to finding an optimal subset repair that may be of independent interest.

==> response.tex <==
\section{Response to Reviewers}

We would like to thank the reviewers for pointing out a bug in the proof of Sublemma 1. The reviewers are correct in that, as presented in the paper, $M$ is not necessarily a matching. However, we will show that we can construct the desired maximal matching by slightly modifying the argument. We should note that the construction of the reduction and the gadgets remain exactly the same as before.

	\begin{figure}[!ht]
	    \centering 
    \begin{tikzpicture}[->,>=stealth,auto=left, semithick,scale=2,vnode/.style={black,inner sep=2pt,scale=1},el/.style = {inner sep=3/2pt}]
      \node[vnode] (c0) at (1,0) {$y^0_j$};
      \node[vnode] (p1) at (1,4/3) {$C_\kappa^+$};
       \node[vnode] (p2) at (3,4/3) {$C_\lambda^+$};
       \node[vnode] (d0) at (1,2/3) {$x_j^0$};
      \node[vnode] (c2) at (2,0) {$y_j^2$};
      \node[vnode] (d2) at (2,2/3) {$x_j^2$};
      \node[vnode] (d1) at (3,2/3) {$x_j^1$};
      \node[vnode] (c1) at (3,0) {$y_j^1$};
      \node[vnode] (m) at (2,4/3) {$C_\mu^-$};

       \path[->] (c0) edge node[el] {0} (c2); 
       \path[->] (c1) edge node[el] {0} (c2); 
       \path[->,densely dotted] (d2) edge node[el] {$1$} (c2);  
       \path[->,densely dashed] (c1) edge node[el] {$1$} (d1);  
	\path[->,densely dashed] (c0) edge node[el] {$1$} (d0);  
	\path[->,densely dashed] (d2) edge node[el] {$1$} (m);  
	\path[->,densely dotted] (p1) edge node[el] {$1$} (d0);
	\path[->,densely dotted] (p2) edge node[el] {$1$} (d1);    

    \end{tikzpicture}	   
	    \caption{Variable gadget for the hardness reduction from the SAT-3-restricted problem.}
	    \label{fig:gadget}
	\end{figure}


\begin{proof}
$\Rightarrow$  Assume that the variable assignment $\psi$ makes $\phi$ satisfiable. {\color{blue} Fix any order of variables $x_1 \dots, x_n$.} We form a set of edges $M$ as follows. For any variable $x_j$ visited in the above order, we distinguish two cases:
%
\begin{itemize} 
\item $\psi(x_j) = \textsf{true}$: we pick $(x_{j}^{2}, y_{j}^{2})$.  If $C_{\kappa}^{+}$ is not yet matched, pick $(C_{\kappa}^{+}, x_{j}^{0})$, {\color{blue} otherwise pick $(y_{j}^{0}, x_{j}^{0})$}. Similarly for $C_{\lambda}^{+}$. 
\item $\psi(x_j) = \textsf{false}$: pick $(y_{j}^{0}, x_{j}^{0})$ and $(y_{j}^{1}, x_{j}^{1})$. If $C_{\mu}^{-}$ is not yet matched, pick $(x_{j}^{2}, C_{\mu}^{-})$, {\color{blue} otherwise pick $(x_{j}^{2}, y_{j}^{2})$.} 
\end{itemize}

By construction, $M$ contains only edges with label 1. 

\smallskip

{\em Claim 1: $M$ is a matching.} {\color{blue} Since $x_j, y_j$ occur only in a variable gadget, they will have at most one adjacent edge from $M$. By construction, each clause $C_\kappa^+, C_\mu^-$ will also have at most one adjacent edge from $M$.}

\smallskip

{\em Claim 2: $M$ is a maximal matching.} First, observe that by our construction, all $x_j^0, x_j^1, x_j^2$ are matched for any $j=1, \dots, n$. Second, notice that if $\psi(x_j) = \textsf{true}$, the edge $(x_{j}^{2}, y_{j}^{2})$ will be chosen; if $\psi(x_j) = \textsf{false}$, the edges $(y_{j}^{0}, x_{j}^{0})$ and $(y_{j}^{1}, x_{j}^{1})$ will be chosen. Thus, the edges $(y_j^0, y_j^2), (y_j^1, y_j^2)$ can not be added to $M$.
%
Finally, consider the edge $(C_i^+, C_i^-)$ corresponding to clause $C_i$.  If there exists a positive literal which satisfies $C_{i}$, {\color{blue} then consider the earliest $x_{j}$ in the linear order of variables. By construction, $(C_i^+, x_j^\nu)$ is in the matching, where $\nu \in \{0,1\}$.} Otherwise, $C_{i}$ is satisfied by a negative literal: {\color{blue} consider the earliest such $x_k$ in the linear order.  Then $(x_{k}^2, C_{i}^{-})$ is in $M$.}
In either case, $(C_i^+, C_i^-)$ cannot be added to increase the size of the matching.
\end{proof}

